Meta-attention for ViT-backed Continual Learning

Continual learning is a longstanding research topic due to its crucial role in tackling continually arriving tasks. Up to now, the study of continual learning in computer vision is mainly restricted to convolutional neural networks (CNNs). However, recently there is a tendency that the newly emerging vision transformers (ViTs) are gradually dominating the field of computer vision, which leaves CNN-based continual learning lagging behind as they can suffer from severe performance degradation if straightforwardly applied to ViTs. In this paper, we study ViT-backed continual learning to strive for higher performance riding on recent advances of ViTs. Inspired by mask-based continual learning methods in CNNs, where a mask is learned per task to adapt the pre-trained ViT to the new task, we propose MEta-ATtention (MEAT), i.e., attention to self-attention, to adapt a pre-trained ViT to new tasks without sacrificing performance on already learned tasks. Unlike prior mask-based methods like Piggyback, where all parameters are associated with corresponding masks, MEAT leverages the characteristics of ViTs and only masks a portion of its parameters. It renders MEAT more efficient and effective with less overhead and higher accuracy. Extensive experiments demonstrate that MEAT exhibits significant superiority to its state-of-the-art CNN counterparts, with 4.0~6.0% absolute boosts in accuracy. Our code has been released at https://github.com/zju-vipa/MEAT-TIL.

==> floats/tab-results.tex <==
\begin{table*}[!t]
\centering
\setlength{\tabcolsep}{8pt}
\begin{tabular}{ll *{8}{r}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{CUB}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Cars}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{FGVC}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{CIFAR}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Wiki}}}
    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Sketches}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Model}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Added}}}
    % & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Trained}}}
    \\
    & & & & & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{100}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Art}}}
    
    & & 
     \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Size}}}
    & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\#params.}}}
    % & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Size}}}
    % & \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\#params.}}}
    \\
    \midrule
    \multirow{5}{*}{CNNs}
    & LwF & 69.58 & 77.03 & N/A & N/A & N/A  &  N/A &  563 & 0.00  \\
    & PPN & 78.94 & 89.21 &  N/A  &  N/A  & 74.94 & 76.35 & 563 & 5.10   \\
    & PackNet & 80.41 & 86.11 &  N/A  &  N/A  & 69.40 & 76.17 & 115 &  0.05 \\
    & Piggyback & 81.59 & 89.62 &  N/A  &  N/A  & 71.33 & 79.91 & 121 & 0.08  \\
    % & XK-FAC & 80.30 & 88.07 & - & - & - & - &  & 123 &   \\
    & CPG & 83.59 & 92.80 &  N/A  &  N/A & 77.15 & 80.33 & 121 & 0.08  \\
    \midrule

    \multirow{8}{*}{DeiT-Ti} &  
    Classifier & 53.49 & 18.47  & 17.91 & 66.85 & 41.42 & 32.60 &  21 &0.00 \\
    % & finetuning &  71.94(\Blue{\small$\downarrow$44.28}) & 65.99(\Blue{\small$\downarrow$45.53}) & 70.00 & 79.16 &  68.04 & 72.03 \\
    % & LwF &  59.03(\Blue{\small$\downarrow$3.01}) & 39.29(\Blue{\small$\downarrow$6.88}) & 38.87(\Blue{\small$\downarrow$5.90}) & 68.79(\Blue{\small$\downarrow$3.14}) \\

    & Finetuning & 71.94 & 65.99 & 70.00 & 79.16 & 68.04 & 72.03 & 21 & 0.00  \\

    & Finetuning$^\dagger$ &  -$44.28$ & -$45.53$ & -$43.44$ & -$13.28$ & -$39.71$ & -$38.91$ & N/A & N/A   \\
    
    & LwF & 59.03 & 39.29 & 38.87 & 68.79 & 46.88 & 53.17 & 21  & 0.00  \\
    & LwF$^\dagger$ & -$3.01$ & -$6.88$ & -$5.90$ & -$3.14$ & -$8.96$ & -$6.06$ & N/A & N/A  \\
    % & EwC & \\
    
    & Piggyback & 60.65 & 44.87 & 45.58 & 71.18 & 62.42 & 69.07 & 21 & 0.02   \\
    & BERT-adaptor & 66.03 & 45.50 & 41.28 & 75.21 & 57.04 & 71.21 & 23 & 0.10  \\
    & Ours & \textbf{69.16} & \textbf{51.42} & \textbf{52.28} & \textbf{77.42} & \textbf{64.25} & \textbf{76.73} & 21 & 0.02   \\
    \midrule
    
    \multirow{8}{*}{DeiT-S}  &
    Classifier & 66.22 & 24.28  & 24.21 & 73.32 & 47.87 & 46.08 & 85 &0.00  \\ 
    % & finetuning & 82.15(\Red{new line}\Blue{\small$\downarrow$39.04}) & 82.29(\Blue{\small$\downarrow$39.22}) & 76.06 & 86.25 & 75.03 & 78.83 \\
    % & LwF & 69.34(\Blue{\small$\downarrow$4.20}) & 74.00(\Blue{\small$\downarrow$6.88}) & 55.99(\Blue{\small$\downarrow$6.12}) & 80.67(\Blue{\small$\downarrow$2.33}) \\

    & Finetuning & 82.15 & 82.29 & 76.06 & 86.25 & 75.03 & 78.83 & 85 &0.00   \\
    
    & Finetuning$^\dagger$ &  -$33.46$ & -$49.46$ & -$40.17$ & -$10.06$ & -$35.93$ & -$29.61$ & N/A & N/A   \\
    
    & LwF & 69.34 & 74.00 & 55.99 & 80.67 & 65.64 & 70.74 & 85 &0.00  \\
    
    & LwF$^\dagger$ & -$3.77$ & -$5.98$ & -$7.09$ & -$2.44$ & -$4.72$ & -$2.53$ & N/A & N/A  \\    
    % & EwC & \\
    & Piggyback & 72.89 & 74.72 & 60.04 & 79.76 & 68.09 & 75.03 & 87 & 0.02   \\
    & BERT-adaptor & 77.20  & 67.23 & 57.04 & 84.46 & 71.33 & 72.87 & 80 & 0.06    \\ 
    & Ours & \textbf{83.34} & \textbf{77.20} & \textbf{64.69} & \textbf{84.89} & \textbf{72.43} & \textbf{77.68} & 87 & 0.02 \\
    \midrule
    
    \multirow{7}{*}{T2T-S}   &
    Classifier & 33.10 & 11.52 & 14.04 & 33.10 & 38.92 & 20.65 & 25 &0.00   \\ 
    % & finetuning & 73.08(\Blue{\small$\downarrow$41.35}) & 73.67 & 64.12 & 73.08 & 69.76 & 76.90 \\
    % & LwF & 45.33(\Blue{\small$\downarrow$2.02}) & 59.01(\Blue{\small$\downarrow$8.11}) & 42.07(\Blue{\small$\downarrow$7.87}) & 70.34(\Blue{\small$\downarrow$2.37})\\
    % & EwC & \\

    & Finetuning & 73.08 & 73.67 & 64.12 & 73.08 & 69.76 & 76.90 & 25 &0.00 \\

    & Finetuning$^\dagger$ &  -$48.90$ & -$53.46$ & -$47.16$ & -$13.99$ & -$42.04$ & -$43.09$ & N/A & N/A \\
    
    & LwF & 45.33 & 59.01 & 42.07 & 70.34 & 51.24 & 61.98 & 25 &0.00    \\

    & LwF$^\dagger$ & -$2.53$ & -$3.51$ & -$9.48$ & -$3.09$ & -$9.76$ & -$8.21$ & N/A & N/A\\    
    
    & Piggyback & 63.57 & 58.22 & 51.47 & 70.98 & 66.34 & 78.07 & 25 & 0.02  \\
    & BERT-adaptor & 64.31 & 53.79 & 48.02 & 73.58 & 59.01 & 74.02 & 28 & 0.12 \\
    & Ours & \textbf{69.90} & \textbf{61.90} & \textbf{53.55} & \textbf{76.42} & \textbf{61.20} & \textbf{73.75} & 25 & 0.02  \\
    
    \bottomrule
\end{tabular}
\caption{Comparison of performance on six new tasks added on the initial ImageNet task between all involved models. Specifically, methods marked with $\dagger$ refer to the forgetting percentage~(\%) on the old ImageNet task. Only Finetuning and LwF methods suffer from forgetting problems here. Bold font indicates the best performance in each vision transformer. ``Size'' denotes model size~(MB). ``Added \#params'' presents the times~($\times$) of increased parameter sizes than a model which only trains a new classifier for studying a new task. Note that for all incremental learning methods, introducing a new classifier is fundamental for the incoming task. We hence leave the parameters of all new classifiers out in statistics of model sizes. For example, Classifier baseline only trains new classifiers and introduces $0.00\times$ parameter size.}
% All datasets are added from left to right, our method is task order-robust.}
\label{tab:results}
\end{table*}

